Model Monitoring in the Absence of Labeled Data via Feature Attributions Distributions

Model monitoring involves analyzing AI algorithms once they have been deployed and detecting changes in their behaviour. This thesis explores machine learning model monitoring ML before the predictions impact real-world decisions or users. This step is characterized by one particular condition: the absence of labelled data at test time, which makes it challenging, even often impossible, to calculate performance metrics. The thesis is structured around two main themes: (i) AI alignment, measuring if AI models behave in a manner consistent with human values and (ii) performance monitoring, measuring if the models achieve specific accuracy goals or desires. The thesis uses a common methodology that unifies all its sections. It explores feature attribution distributions for both monitoring dimensions. Using these feature attribution explanations, we can exploit their theoretical properties to derive and establish certain guarantees and insights into model monitoring.

==> content/RelatedWork.tex <==
\chapter{Literature Review} \label{c2}

\section{Model Monitoring Under Distribution Shift}

\subsection{Detecting Distribution Shift and its Impact on Model Behaviour:}

A lot of related work  has aimed at detecting that data is from out-of-distribution. To this end, they have created several benchmarks that measure whether data comes from in-distribution or not~\cite{wilds,wilds_ext,malinin2021shifts,malinin2022shifts,DBLP:conf/nips/MalininBGGGCNPP21}. In contrast, our main aim is to evaluate the impact of the distribution shift on the model. A typical example is two-sample testing on the latent space such as described by Rabanser et al.~\cite{DBLP:conf/nips/RabanserGL19}. However, many of the methods developed for detecting out-of-distribution data are specific to neural networks processing image and text data and can not be applied to traditional machine learning techniques. These methods often assume that the relationships between predictor and response variables remain unchanged, i.e., no concept shift occurs. Our work is applied to  tabular data where techniques such as gradient boosting decision trees achieve state-of-the-art model performance~\cite{grinsztajn2022why,DBLP:journals/corr/abs-2101-02118,BorisovNNtabular}. 

 
Evaluating how two distributions differ has been a widely studied topic in the statistics and statistical learning literature~\cite{statisticallearning,datasetShift,DBLP:conf/icml/LiuXL0GS20} and  has advanced in recent years ~\cite{DBLP:conf/nips/ParkAKP21,DBLP:conf/nips/LeeLLS18,DBLP:conf/icml/ZhangSMW13}. The use of supervised learning classifiers to measure statistical tests has been  explored by Lopez-Paz et al.~\cite{DBLP:conf/iclr/Lopez-PazO17} proposing a classifier-based approach that returns test statistics to interpret differences between two distributions. We adopt their power test analysis and interpretability approach but apply it to the explanation distributions.


\subsection{Impossibility of Model Monitoring} 
Recent research findings have formalized the limitations of monitoring machine learning models in the absence of labelled data. Specifically~\cite{garg2022leveraging,chen2022estimating} prove the impossibility of predicting model degradation or detecting out-of-distribution data with certainty~\cite{fang2022is,DBLP:conf/icml/ZhangGR21,guerin2022outofdistribution}. Although our approach does not overcome these limitations, it provides valuable insights for machine learning engineers to understand better changes in interactions resulting from shifting data distributions and learned models.


\subsection{Model Monitoring and Distribution Shift Under Specific Assumptions}
Under specific types of assumptions, model monitoring and distribution shift become feasible tasks. One type of assumption often found in the literature is to leverage causal knowledge to identify the drivers of distribution changes~\cite{DBLP:conf/aistats/BudhathokiJBN21,zhang2022why,schrouff2022diagnosing}. For example, Budhathoki et al.~\cite{DBLP:conf/aistats/BudhathokiJBN21} use graphical causal models and feature attributions based on Shapley values to detect changes in the distribution.
%\steffen{Let us assume we provided a naive (though wrong) causal model that would causally connect, e.g., every attribute to the target variable. Would their approach then become equivalent to our approach?}\carlos{I don't understand this}
Similarly, other works aim to detect specific distribution shifts, such as covariate or concept shifts.  Our approach does not rely on additional information, such as a causal graph, labelled test data, or specific types of distribution shift. Still, by the nature of pure concept shifts, the model behaviour remains unaffected and new data need to come with labelled responses to be detected.


\subsection{Explainability and Distribution Shift}

Lundberg et al.~\cite{lundberg2020local2global} applied Shapley values to identify possible bugs in the pipeline by visualizing univariate SHAP contributions. In our work we go beyond debugging and formalize the multivariate explanation distributions where we perform a two-sample classifier test to detect distribution shift impacts on the model. Furthermore, we provide a mathematical analysis of how the SHAP values contribute to detecting distribution shift. 

Another approach using Shapley values by Balestra et al.~\cite{li2022enabling} allows for tracking distributional shifts and their impact among for categorical time series using slidSHAP, a novel method for unlabelled data streams. In our work, we define the explanation distributions and exploit its theoretical properties under distribution shift where we perform a two-sample classifier test to detect 


Haut et al.~\cite{haug2021learning} track changes in the distribution of model parameter values that are directly related to the input features to identify concept drift early on in data streams. In a more recent paper,Haug et al.~\cite{haug2022change} also exploits the idea that local changes to feature attributions and distribution shifts are strongly intertwined and uses this idea to update the local feature attributions efficiently. Their work focuses on model retraining and concept shift, in our work the original estimator $f_\theta$ remains unaltered, and since we are in an unsupervised monitoring scenario we can't detect concept shift see discussion in Section \ref{sec:discussion}

\section{Fairness}\label{sec:relatedWork}

\subsection{Fairness and Auditing}


\enquote{Audits are tools for interrogating complex processes, often to determine whether they comply with company policy, industry standards or regulations}~\citep{DBLP:conf/fat/RajiSWMGHSTB20}. Algorithmic fairness audits are closely linked to audits studies as understood in the social sciences, with a strong emphasis on social justice~\citep{DBLP:conf/eaamo/VecchioneLB21}. A recent survey on public algorithmic audit identified four categories of \enquote{problematic machine behaviour} that can be unveiled by audit studies: discrimination, distortion, exploitation and misjudgement \citep{DBLP:journals/pacmhci/Bandy21,liu2012enterprise}. This taxonomy is highly helpful when putting forward auditing studies and also relevant for this work: our \enquote{Equal Treatment Inspector} can be seen as a tool to help understand discrimination in machine learning models, thus, falling into the first category.


Selecting a measure to compare fairness between two sensitive groups has been a highly discussed topic, where results such as~\citep{DBLP:journals/bigdata/Chouldechova17,DBLP:conf/nips/HardtPNS16,DBLP:conf/innovations/KleinbergMR17}, have highlighted the impossibility to satisfy simultaneously three type of fairness measures: demographic parity~\citep{DBLP:conf/innovations/DworkHPRZ12}, equalized odds~\citep{DBLP:conf/nips/HardtPNS16}, and predictive parity~\citep{DBLP:conf/kdd/Corbett-DaviesP17,DBLP:journals/corr/abs-2102-08453,wachter2020bias}. Previous work has relied on the notion of equal outcomes by measuring and calculating demographic and statistical parity on the model predictions \citep{kearns2018preventing}.
The arguments of ~\cite{DBLP:conf/aies/SimonsBW21} provide background and motivation towards interpretations of equal treatment as blindness and discuss its importance in practical policy applications. 


\subsection{Explainability for Fair Supervised Learning}

The intersection of fairness and explainable AI has been an active topic in recent years. The most similar work is ~\citep{lundberg2020explaining} where they apply Shapley values to statistical parity.
Our work continues in-depth on this research line by formalizing the explanation distribution, deriving theoretical guarantees, and proposing novel methodology. Specifically, our approach allows for comparison across different protected groups. We also introduce the concept of accountability, which refers to the ability of the algorithm to provide insights into the sources of \emph{equal treatment} violation of the model. Additionally, we evaluate our method on multiple datasets and synthetic examples, demonstrating its effectiveness in identifying and mitigating equal treatment disparities in machine learning models.


A recent line of work assumes knowledge about causal relationships between random variables. For example,~\cite {DBLP:conf/fat/GrabowiczPM22} presents a post-processing method based on Shapley values aiming to detect and nullify the influence of a protected attribute on the output of the system. They assume known direct causal links from the data to the protected attribute and no measured confounders. Our work does not rely on causal graphs knowledge but exploits the Shapley values' theoretical properties to obtain fairness model auditing guarantees. 

~\cite{DBLP:conf/ssci/StevensDVV20} presents an approach to explaining fairness based on adapting the Shapley value function to explain model unfairness. They also introduce a new meta-algorithm  that considers the problem of learning an additive perturbation to an existing model in order to impose fairness. 
In our work, we do not adopt the Shapley value function. Instead, we use the theoretical Shapley properties to provide fairness auditing guarantees. Our \textit{Equal Treatment Inspector} is not perturbation-based but uses Shapley values to project the model to the explanation distribution, and then measures \emph{un-equal treatment}. It also allows us to pinpoint what are the specific features driving this violation.
 
 
In ~\cite{DBLP:conf/fat/GrabowiczPM22}, the authors present a post-processing method based on Shapley values aiming to detect and nullify the influence of a protected attribute on the output of the system. For this, they assume there are direct causal links from the data to the protected attribute and that there are no measured confounders. Our work does not use causal graphs but exploits the theoretical properties of the Shapley values to obtain fairness model auditing guarantees.

Instead of using feature attribution explanation, other works have researched fairness using other explainability techniques such as counterfactual explanations \citep{DBLP:conf/nips/KusnerLRS17,DBLP:conf/cogmi/ManerbaG21,DBLP:conf/aies/MutluYG22}.
We don't focus on counterfactual explanations but on feature attribution methods that allow us to measure unequal feature contribution to the prediction. Further work can be envisioned by applying explainable AI techniques to the \enquote{Equal Treatment Inspector} or constructing the explanation distribution out of other techniques.


\subsection{Classifier Two-Sample Test}
The use of classifiers to obtain statistical tests or measure independence between two distributions has been previously explored in the literature \citep{DBLP:conf/iclr/Lopez-PazO17}. Specifically, the first authors introduced the use of \enquote{Classifier Two-Sample Tests (C2ST)} to represent the data that returns an interpretable unit test statistic, allowing it to measure how two distributions differ from each other. Their approach establishes the main theoretical properties, compares performance against state-of-the-art methods, and outlines applications of C2ST. 
Similar work of~\cite{DBLP:conf/icml/LiuXL0GS20} propose a kernel-based to two-sample
tests classification, aiming to determine whether two samples are drawn from the same underlying distribution. 
Alike work has also been used in Kaggle competitions under the name of \enquote{Adversarial Validation}~\citep{kaggleAdversarial,howtowinKaggle}, a technique which aims to detect which features are distinct between train and leaderboard datasets to avoid possible leaderboard shakes. 
Our work builds on previous approaches by adopting their interpretable power test analysis and theoretical properties. Still, we focus on testing for fairness notions of equal treatment in the explanation distribution. As the test statistic for our approach, we use the Area Under the Curve (AUC) of the \enquote{Equal Treatment Inspector}.

Another related work in the literature is by \cite{DBLP:journals/corr/EdwardsS15}, who focuses on removing statistical parity from images by
using an adversary that tries to predict the relevant sensitive variable from the model representation and censoring the learning of the representation of the model and data on images and neural networks. While methods for images or text data are often developed specifically for neural networks and cannot be directly applied to traditional machine learning techniques, we focus on tabular data where techniques such as gradient boosting decision trees achieve state-of-the-art model performance \citep{DBLP:conf/nips/GrinsztajnOV22,DBLP:journals/corr/abs-2101-02118,BorisovNNtabular}. 
Furthermore, our model and data projection into the explanation distributions leverages Shapley value theory to provide fairness auditing guarantees. In this sense, our work can be viewed as an extension of their work, both in theoretical and practical applications.



==> content/data/analysis.tex <==
\section{Data Assessment Matrix}\label{sec:analysis}

%Figure \ref{fig:datamatrix} summarises the proposed data analysis dimensions (see Section~\ref{data_dim}) and their categorisation.


 \begin{figure}[ht]
     \centering
 \includegraphics[width=1\textwidth]{content/data/images/ATI_Data_Matrix.pdf}
     \caption{Summary data assessment matrix for the five data dimensions proposed in this paper.}
     \label{fig:datamatrix}
 \end{figure}

%\textcolor{red}{Should the section header be data assessment matrix? This is what is referenced to in Section 5}\carlos{Prob}


\subsection{Appropriateness: Is the data relevant to the questions posed?}
Data appropriateness refers to how relevant the data is for the challenge or research questions at hand:

%\begin{itemize}
\textit{Insufficient:} Data is not related to the challenge question or is completely unrelated to the problem at hand. As an example, a datathon team is tasked with predicting consumer behavior for a new product launch but is given data on historical weather patterns instead.
    
\textit{Developing:} Data is related to the challenge question, but the target variables needed to answer the research questions are missing. For example, a datathon may seek to predict stock price movements from historical transaction data but without stock  prices, it would be challenging to produce useful results.

\textit{Functional:} Data is appropriate for the challenge but the features can notably be enhanced with data the partner organisation could provide. For example, a datathon team is given a dataset on website traffic and user behavior, which is relevant to their challenge, but they identify that additional data on customer feedback would be helpful in making more accurate predictions.
    
\textit{Optimal:} Data is highly appropriate and relevant to the challenge. A datathon team is given comprehensive datasets which provide all the necessary information for making accurate predictions and developing effective solutions. Appropriate meta-data and collection processes are also provided.

    
%\end{itemize}

\subsection{Readiness: Is the data analysis ready?}

% Do we want to add more details here? 

Data readiness refers to the degree to which data is prepared and available in a datathon. This includes factors such as the quality and completeness of the data, the availability of relevant metadata, and the ease with which the data can be accessed and analysed. Ease and effectiveness of analysis are closely coupled to effective and thorough data documentation \citet{DBLP:journals/cacm/GebruMVVWDC21,DBLP:journals/corr/abs-1805-03677}, which increase transparency, understandability, and accountability of data and model usage~\citep{DBLP:conf/fat/MitchellWZBVHSR19}. Data readiness categories are as follows:


\textit{Insufficient:} No data has been collected yet, and there is no methodology for doing so. For example, if the datathon involves collecting data from sensors, and there isn't a clear view of where the data is being stored or what it actually contains, the data readiness degree would be \emph{insufficient}.

\textit{Developing:} Some data has been collected, and a firm methodology is in place for doing so. However, there may still be some uncertainty around its quality and completeness. For example, if the datathon involves analysing customer data from a company, and even though they have access to their data, parts of it are missing, 
 or inconsistent, the data readiness degree would be \emph{developing}.

\textit{Functional:} Data is collected, but some merging and unifying still need to be done during the event. The data may require some cleaning and preprocessing, but with minor processing can serve to answer the challenge questions. For example, if the datathon involves analysing public transportation data from different sources, and some data needs to be merged, aggregated, and formatted to fit into the analysis, the data readiness degree would be \emph{functional}.

\textit{Optimal:}  Data is collated, clean, with no missing gaps, and can potentially be fed to a learning algorithm with minimal processing. The data is also documented with the data dictionary and data cards, such as the ones highlighted in previous research ~\citep{DBLP:journals/cacm/GebruMVVWDC21,pushkarnaDataCardsPurposeful2022} but in the context of datathons.  It is worth noting that dataset documentation in general remains a developing field of study, and datathon-specific recommendations or guidelines are yet to be established.  For example, if the datathon involves analysing a well-established dataset, such as the MNIST dataset, the data readiness degree would be \emph{optimal}.



\subsection{Reliability: How biased is the data?}

 Reliability here refers to the extent to which the data accurately represents the population or phenomenon without systematic data collection errors or distortions. 

\textit{Insufficient:} Data has significant known biases, and conclusions drawn from the analysis will be undermined. For example, in a datathon studying democratic voting patterns, the dataset only includes responses from a small, self-selected group of participants, rendering it insufficient to make accurate inferences about the broader population's voting behavior.
    
\textit{Developing:} Data has unknown or indeterminate roots of bias, and hence no firm conclusions can be made using only these data sources. For example, in a datathon analysing economic indicators of different countries, it is suspected that there are geographical and temporal inconsistencies in the data collection. As a result, the dataset is considered to be in the \emph{developing stage} of reliability.

\textit{Functional:} Data has known biases that will impact the analysis and can be corrected or accounted for as a work limitation. For example, in a datathon analysing customer feedback surveys, it is known that the surveys were only completed by customers who voluntarily provided feedback, introducing a self-selection bias. The organisers acknowledge this limitation and proceed with the analysis, highlighting the potential impact of the bias on the conclusions.
    
\textit{Optimal:} Data does not suffer from a known source of biases with significance for the conclusions. For example, in a datathon exploring climate change impacts, the dataset comprises meticulously collected climate measurements from a comprehensive network of sensors across multiple regions. 

\subsection{Sensitivity: Is the data private or confidential?}

Data sensitivity refers to the level of confidentiality and privacy associated with specific types of data. It indicates the degree to which the data is considered private, personal, or valuable, requiring enhanced protection. Ensuring these safeguards may increase the difficulty of hosting a datathon. Therefore, we map the sensitivity tiers described by~\cite{DBLP:journals/corr/abs-1908-08737} to our analysis framework.

%\carlos{Change insufficient for prohibit, and developing for challenging? Better not to break the flow.}

\textit{Insufficient (Tier 4):} Highly sensitive data presents significant threats, making hosting a datathon impractical. Due to potential legal and personal risks, datathons are not supported at this tier. For instance, handling datasets with commercial or national security sensitivities. This aligns with the UK government's \enquote{\textit{secret}} classification \citep{ukcabinetoffice}. At Tier 4, the risk of malicious actors infiltrating the datathon team becomes notable.

\textit{Developing (Tier 3):} Careful consideration and extensive security measures would be required prior to hosting a datathon in this tier. Datathon participants would be restricted in their use of tools, location and network connections, increasing system friction. For example, in a medical context, a dataset containing highly sensitive patient health records, including names, addresses, and detailed medical histories, poses a substantial threat
    
\textit{Functional (Tier 2):} Data in this tier does not present significant personal, legal or commercial risk. However, sufficient measures must be taken to mitigate processing risks, such as \emph{(i)} data de-anonymisation, \emph{(ii)} competitive data leakage \emph{(iii)} or inadvertent disclosure. These measures increase the difficulty of participants interacting with the data. For example, an educational dataset with anonymized student records that still hold the risk of re-identification. Hosting a datathon using this data would necessitate robust security measures to prevent any potential breach of student privacy and unauthorized access to sensitive academic information.

\textit{Optimal (Tier 0/1):} Since risks associated with this data are limited, hosting datathons in virtual environments is usually unnecessary. Free data access to the participants reduces system friction. A dataset containing weather records from a public weather station that doesn't include any personal or sensitive information would fall under this tier. 


More details, including a discussion on the classification process, as well as the technical requirements to build such environments can be found in \citep{DBLP:journals/corr/abs-1908-08737}.

\subsection{Sufficiency: How much data is enough data for a given datathon?}

Data sufficiency refers to the quantity of available data to investigate the challenge questions given a proposed approach. In addition to case-by-case (e.g., depending on the approach and the question) considerations, we propose below an assessment based on previous experiences of similar challenges. In section \ref{case_studies}, which is problem-specific, we make case-specific comments on data sufficiency. 


\textit{Insufficient}: Prior experiences have shown that working with similar data quantities on projects with similar objectives hinders the overall success and outcomes of the datathon. For example,  in a medical research datathon aiming to predict patient outcomes, the provided dataset does not include information about clinical trials. 


\textit{Developing}: Prior experience has shown that the quantity of data available is not substantial enough to address the research question comprehensively. This quantity of data raises questions about its ability to offer statistical evidence and comprehensive insights into the challenge questions, unlike the \textit{insufficient} category, data may be present but not adequate for comprehensive insights. For example, a dataset containing a few time-series signals in an industrial failure detection manufacturing datathon not allowing to distinguish between normal and failure modes~\citep{amrc22}.

\textit{Functional}: Although not surpassing previous successful datathons, prior experience has shown that the quantity of data is sufficient to provide useful insights and statistical evidence into the challenge questions. Any insufficiency can be accounted for as a work limitation and discussed in future work. For example, in a datathon focused on developing an automated system for classifying sea ice and mapping seals to aid ecological monitoring, the geospatial data provided covered only two focal areas, which limits the potential generalizability of the developed system to broader regions~\citep{data-study-group-antarctic}.

\textit{Optimal}: This category represents an amount of data which surpasses previous successful datathons. The dataset(s) is extensive (potentially more than what was proposed initially), offering a rich source of information for participants to explore and leverage as they tackle the challenge questions.  For example, in a datathon that aims to predict the functional relationship between DNA sequence and the epigenetic state, having access to  comprehensive and well-labelled genomic datasets~\citep{dsg-dementia-report}.


==> content/data/cases.tex <==
\section{Case Studies}\label{sec:casestudies}
\label{case_studies}

We evaluated the quality of data in past DSGs
%(Data Study Group) 
by referring to the final reports available on The Alan Turing Institute's website\footnote{\url{https://www.turing.ac.uk/collaborate-turing/data-study-groups}} and show an aggregate summary of the results in Figure~ \ref{fig:heatmap}. It is important to acknowledge a publication bias in these reports, as only those that meet minimum quality criteria determined by the reviewing team are made available. Moreover, the reports from early DSGs might not have been published due to problems ranging from unresolved sensitivity issues to misaligned expectations between organisers and challenge owners. Consequently, our focus was primarily on the later versions of the DSG.


This section presents the ten most recent datathons case studies, selected from over 80 datathons, in Figure~\ref{fig:heatmap} we provide a summary of the results of the data assessment of the case studies. These case studies have data, challenge descriptions, and  limitations extracted from the publicly available DSG Reports. 

\begin{figure}[ht]
    \centering
\includegraphics[width=0.8\textwidth]{content/data/images/heatmap.pdf}
    %\caption{Classification of the latest 10 DSG reports based on the data assessment matrix proposed in this paper, showing report counts. Note that we shortened ``appropriateness'' to ``appropriate'' and ``readiness'' to ``ready'' for space.}
    \caption{Report count data assessment classification of the last 10 DSG reports}
    \label{fig:heatmap}
\end{figure}

\subsection{Cefas: Centre for Environment, Fisheries and Aquaculture Science}\label{case:cefas}
The datathon aimed to address the challenge of automating the classification of plankton species and detritus in millions of images collected by the Cefas Endeavour research vessel's Plankton Imager system, enabling efficient analysis and contributing to the understanding and conservation of marine ecosystems~\citep{cefas2022}.

\textbf{Appropriateness. }\textit{(Optimal)} Plankton images and their corresponding labels were present in the data: \enquote{expert manual classification (labels) allowed challenge participants to verify the accuracy of the automated classification methods explored.}

\textbf{Readiness.} \textit{(Functional)} Images had faulty labels: \enquote{[\ldots] we discovered that a number of the images labelled as detritus were in fact empty.}

\textbf{Reliability. }\textit{(Optimal)} When writing the challenge proposal, we identified a potential bias in the data collection method: all images were collected by the same imager system on the same vessel.  However, Cefas did not assess this risk as substantial, which was corroborated by the project outcome.

\textbf{Sensitivity. }\textit{(Optimal)} The data is open access, collected by the Plankton Imager\footnote{\url{ https://data.cefas.co.uk/view/20507}}.

\textbf{Sufficiency.} \textit{(Functional)} Some species of plankton were under-represented, making it an imbalanced problem which needed to be accounted for in the analysis (e.g. using data augmentation).



\subsection{The University of Sheffield Advanced Manufacturing Research Centre: Multi-sensor based Intelligent Machining Process Monitoring}\label{case:sheffield}

% Can condense this description later
This challenge aimed to enhance process monitoring in modern manufacturing using machine learning techniques to analyse multiple sensor measurements~\citep{amrc22}. Two datasets were provided for this challenge containing
time-series process signals of the machine operating in both normal and
failure modes. The datasets were recorded during separate machining
trials.

\textbf{Appropriateness.} \textit{(Developing)} The target variables needed for the challenge were not present in the data: \enquote{the provided dataset does not contain any data describing the transition period between the normal operation mode and failure modes}

\textbf{Readiness.} \textit{(Functional)} The data requires aggregation before being used: \enquote{datasets were collected at extremely
high sampling frequencies \ldots resulted in excessively big datasets}

\textbf{Reliability.} \textit{(Functional)} The data experiments were not recorded in the same instance so although measures were taken to ensure that they were as identical as possible, there was a known bias that could be accounted for: \enquote{The two provided datasets were recorded during two separate machining trials [...]. However, a number of identical components were machined in each trial to act as repeats for the dataset.}

\textbf{Sensitivity.} \textit{(Functional)} The data was commercially sensitive and was mapped as Tier 2.

\textbf{Sufficiency.} \textit{(Developing)} Not enough data for the analysis: \enquote{There were still not enough multivariate time series produced by different runs of the experiment to accurately use image classification.}



\subsection{CityMaaS:  Making Travel for People in Cities Accessible through Prediction and Personalisation}\label{case:citymaas}

The aim of this datathon was to develop a platform that provides reliable information on the accessibility of destinations \citep{data-study-group-citymaas}. In particular, participants were tasked to $(i)$ predict the accessibility of points of interest (POIs) in a city; $(ii)$ to develop a personalised route-planning algorithm with accessibility constraints and for different \enquote{persona} types of their users. For $(i)$, CityMaaS provided manually enhanced point data from OpenStreetMap (OSM) \citep{OpenStreetMap} and for $(ii)$ information on (synthetic) potential end-user personas were provided (i.e. place of residence, civil status, profession, income, conditions, etc.).


\textbf{Appropriateness.} \textit{(Developing)} The enhanced OSM dataset provided for the task $(i)$ was appropriate for predicting POI accessibility. However, for task $(ii)$, participants were only given information about the profile of potential users. 

\textbf{Readiness.} \textit{(Functional)} Significant data cleaning was necessary before the analysis was performed; for example, participants noted the need to \enquote{homogenise} the POI data to avoid naming errors in the dataset.

\textbf{Reliability.} \textit{(Developing)} The dataset for POI prediction had a class imbalance with 73\% of POIs being labelled as accessible. POI data was taken from OSM where users are allowed to input tags leading to possible errors and annotation bias.

\textbf{Sensitivity.} \textit{(Functional)} There was commercial sensitivity for CityMaaS in providing the enhanced OSM dataset provided and the (synthetic) user profiles.

\textbf{Sufficiency.} \textit{(Developing)} In particular, for the routing task, no routing data was provided. Participants searched for additional open-source data sources to supplement the data provided by CityMaaS. 


\subsection{WWF: Smart Monitoring for Conservation Areas}\label{case:wwf}

The datathon focused on developing a NLP  system to automatically detect news articles reporting emerging threats to protected areas, enabling real-time monitoring and proactive conservation efforts by WWF and the wider conservation community~\citep{data-study-group-wwf}. The dataset contained  approximately 45,000 files describing news stories relevant to UNESCO World Heritage Sites, of which 135 were labeled as 0-'No threat', 1-'Threat detected but not actors' and 2-'Threat with actors'.

\textbf{Appropriateness.} \textit{(Optimal)} The data was obtained using the Google News API and was manually labeled by  WWF experts to be relevant to the challenge.

\textbf{Readiness.} \textit{(Developing)} Even thought there was a data collection methodology in place, the team had to increase the number of data  points available during the event: \enquote{\ldots this dataset was expanded during the DSG week to 1,000 labelled data points}.

\textbf{Reliability.} \textit{(Functional)} Data was manually labelled by WWF experts and scraped using the Google News API, creating a before-hand known data collection bias.

\textbf{Sensitivity.} \textit{(Optimal)} News articles were scraped using Google News API which made it an open source project of Tier 0. 

\textbf{Sufficiency.} \textit{(Developing)} The number of news scraped was potentially sufficient, but the amount of labeled data was insufficient: \enquote{\ldots initially a training dataset of 135 news articles annotated by the WWF experts were supplied}.

\subsection{British Antarctic Survey: Seals from Space}

The datathon aimed to create an automated system for classifying sea ice, mapping seals, and exploring environmental factors to facilitate ecological monitoring and understanding of the Antarctic ecosystem~\citep{data-study-group-antarctic}. The data consisted of GeoTIFF files covering two focal areas, the Antarctic Peninsula (Crystal Sound and Marguerite Bay) and Signy Island. Location data from over 2000
manually-counted seals accompanied these images. 

\textbf{Appropriateness.} \textit{(Functional)} Even though the images and seal location data were provided, some important  covariates such as nursing locations, ice features, or marine food availability, were not provided. 

\textbf{Readiness.} \textit{(Optimal)}  Data was in an appropriate state to apply learning algorithms.

\textbf{Reliability.} \textit{(Functional)} Data collection bias since seal counting has only been attempted on some regions: \enquote{as we do not have image scenes of locations in which counting has been attempted but zero seals have been observed, we cannot generalise our results to other regions of ice}.

\textbf{Sensitivity.} \textit{(Optimal)} The data was open source and classified at Tier 1.

\textbf{Sufficiency.} \textit{(Functional)} The variability on spatial points was restricted to two locations representing typical seal communities. In order to properly validate the model, it should be done by statistical testing in  a new region outside of the given ones.

\subsection{DWP: Department for Work and Pension}

The UK Department of Work and Pensions (DWP) processes a large amount of personal data, including demographics, family circumstances, and financial details, which presents opportunities for large-scale data analysis and concomitant risks to personal privacy. This datathon \citep{deinehaDataStudyGroup2021} evaluated the potential for generating synthetic instances from the original data while preserving utility.  
The DWP provided two datasets of Universal Credit claimant data. Both datasets were synthetic data, representing the original sensitive population, and are close in structure to existing DWP datasets.

\textbf{Appropriateness.} \textit{(Optimal)} Since the challenge regarding the evaluation of the similarity of generated datasets, the provided target data and comparator-generated sets were highly appropriate to this task.

\textbf{Readiness.} \textit{(Functional)} Additional cleaning and merging of the target datasets was necessary before processing; secondary datasets required alignment work. 

\textbf{Reliability.} \textit{(Optimal)} Sources of bias in the data collection methodology were identified due to the generation mechanisms for the target dataset. However, these were limited in their effect on the evaluation metrics used.

\textbf{Sensitivity.} \textit{(Functional)} While the target data did not contain real personal identifiers, it was still considered confidential and a potential vector for data breaches. 

\textbf{Sufficiency.} \textit{(Optimal)} A large number of available target data rows exceeded the scope of previous challenges in synthetic data generation.

\subsection{Dementia Research Institute and DEMON Network: Predicting Functional Relationship between DNA Sequence and the Epigenetic State}

This datathon aimed to improve regulatory genomic predictions to understand the impact of genetic variants on gene expression and regulation in disease-relevant cell types, with a focus on dementias such as Alzheimer's disease, and potential implications for drug target development.\citep{dsg-dementia-report}. Four different datasets were provided, containing information about the DNA sequence and the associated chromatin states.

\textbf{Appropriateness.} \textit{(Optimal)} The data provided contained the features and labels of interest. For example, \enquote{\ldots the outputs are always trained to predict one of two epigenetic signals \ldots in 3 cell types}.

\textbf{Readiness.} \textit{(Functional)} Data required merging and aggregating between datasets to be able to extract insights \enquote{Most of the samples were provided with associated DNase-seq data [\ldots] some cell lines [\ldots] were provided with ATAC-seq data instead. Although both assays are broadly used to}

\textbf{Reliability.} \textit{(Functional)} The datasets used were open-source and annotated by domain experts. Some examples of the datasets used were: EpiMap\footnote{\url{http://compbio.mit.edu/epimap/}} and Human Genome 38\footnote{\url{https://www.ncbi.nlm.nih.gov/assembly/GCF_000001405.39}} There were some gaps in the data which the authors were not able to account for. For example, \enquote{All profile data \ldots included occasional not a
number (NaN) values.}

\textbf{Sensitivity.} \textit{(Optimal)} The datasets used were open-source and was mapped to tier 0.

\textbf{Sufficiency.} \textit{(Optimal)} 4 well-labelled and large genomic datasets were used for the challenge.

\subsection{Automating Perfusion Assessment of Sublingual Microcirculation in Critical Illness}

This challenge sought to determine if a validated measure of microcirculatory perfusion, specifically the microcirculatory flow index, can be directly predicted from a video sequence obtained through darkfield microscopy. The goal is to enable automatic, real-time analysis of the videos, reducing the labour-intensive manual analysis process and facilitating the integration of microcirculatory targets into clinical trials for better patient outcomes~\citep{dsgBirm22}. The data comprised 800 grayscale videos of different lengths and
the quality obtained via DFM from 52 patients monitored over four days

\textbf{Appropriateness.} \textit{(Optimal)} The obtained data and labeled was specifically designed for the challenge. \enquote{These videos have been manually analysed to obtain perfusion parameters per short clip, labelling each data point\ldots}

\textbf{Readiness.} \textit{(Functional)} The dataset was ready but required minor renaming, merging and feature extraction.

\textbf{Reliability.} \textit{(Functional)} There were cases in which a video had no perfusion parameters and vice versa. \enquote{some mismatches were identified \ldots cases in which a video had no perfusion parameters and vice versa}.

\textbf{Sensitivity.} \textit{(Functional)} The data was commercially sensitive due to containing videos from patients and was mapped to a Tier 2.

\textbf{Sufficiency.} \textit{(Developing)} Since the data relied on manual labeling, the total amount of data was not sufficient to provide  statistical validity for the method.\enquote{[\ldots]dataset is comprised of a smaller number[\ldots]} 

\subsection{Entale: Recommendation Systems for Podcast Discovery}

The datathon aimed to develop methods for capturing relationships between podcasts, incorporating information about the content discussed within them and using this information to produce podcast recommendations \citep{data-study-group-entale}. The data provided included user data (episode and show listened by the users) and podcast data (episode transcripts and show descriptions).

\textbf{Appropriateness.} \textit{(Optimal)} Since the challenge was to analyse podcast episode content and to produce episode recommendations, user history and podcast data (episode transcripts, episode and show meta-data) is highly appropriate.

\textbf{Readiness.} \textit{(Functional)} Merging and cleaning of the two datasets was necessary before analysis.

\textbf{Reliability.} \textit{(Functional)} Bias was induced by a small overlap between datasets, and since the participants were tasked with producing a recommender system, they had some measurement bias when evaluating their methodology since they should be evaluated with new data.

\textbf{Sensitivity.} \textit{(Functional)} Data was provided by Entale, and so there was a commercial risk for the data.

\textbf{Sufficiency.} \textit{(Functional)} The two datasets provided were large and enabled users to tackle the research question, but the overlap between user episodes listened to, and episode transcripts was only 10\% making it challenging to incorporate user data with detailed episode content fully.

\subsection{Odin Vision: Exploring AI Supported Decision Making for Early-Stage Diagnosis of Colorectal Cancer}

Odin Vision is a UK company that has developed AI technology for detecting and characterising bowel cancer. The aim of this datathon was to explore methods that enhance the explainability of Odin-Vision’s current machine learning models to aid clinical decision-making by (i) adding a measure of predictive uncertainty along with class prediction, (ii) making the classifications more understandable to the clinicians, and (iii) exploring methods that can automatically learn representations of features using generative models~\citep{odinvision2021}. The provided data collated three public datasets of colorectal polyp images, obtained by merging data from white light endoscopy and narrow-band-imaging light sources.

\textbf{Appropriateness.} \textit{(Functional)} A total of three image datasets were employed. Two of them were publicly available and contained both labelled and unlabelled images. The third one was a high-quality, non-public dataset that was not made available to the datathon participants but was employed by Odin Vision to train the models developed during the datathon.


\textbf{Readiness.} \textit{(Developing)} Many of the images from the publicly available datasets were of low quality due to blur and the presence of reflective spots. A considerable number of images had to be either removed or pre-processed in order to alleviate this issue.

\textbf{Reliability.} \textit{(Developing)} In addition to the positive-case bias resulting from unbalanced classes (see section on Sufficiency), the datathon participants concluded that the best approach was to train the models predominantly on Odin Vision's higher quality, non-public dataset, and to use a test set from the publicly available images. As the train and test sets were not drawn from the same distribution, the reported quantitative results might be affected by the distributional shift between the train and test datasets.

\textbf{Sensitivity.} \textit{(Optimal)} The datathon participants only had access to open-source datasets and not to Odin Vision's non-public data, which made this a Tier 0 challenge.

\textbf{Sufficiency.} \textit{(Functional)} Due to the nature of the datasets (real-world medical images), these were relatively small,  with even fewer positive labelled data, which resulted in an insufficient amount of data for learning algorithms and drawing statistically significant answers.

==> content/data/conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}
In this chapter of the thesis, we have analysed data in the context of datathons along five key dimensions: \textit{appropriateness}, \textit{readiness}, \textit{reliability}, \textit{sensitivity} and \textit{sufficiency}. We then mapped 10 case studies from Data Study Groups to our framework and provided a set of recommendations based on the lessons learned. By doing so, we hope to improve the handling of data for organisations prior to datathon events.

Our proposed qualitative analysis provides a degree of data status across several perspectives; these degrees can be adapted or extended, similar to the Technology Readiness Levels provided by NASA~\citep{sadin1989nasa}, which have been extended through time and further work.

==> content/data/data.tex <==
\section{Data Used in this Thesis}


\subsubsection{Datasets.} 

\carlos{Need to rethink about this.}
\carlos{Update and extend} In the main body of the paper we base our comparisons on the UCI Adult Income dataset~\cite{Dua:2019} and on synthetic data. In the Appendix, we extend experiments to several other datasets, which confirm our findings: ACS Travel Time~\citep{ding2021retiring}, ACS Employment, Stackoverflow dataset~\citep{so2019}.
\paragraph{ACS Income}
\paragraph{ACS Mobility}

\paragraph{StackOverflow Survey Data} The dataset used is the StackOverflow annual developer survey, which has over 70,000 responses from over 180 countries examining aspects of the developer experience~\cite {so2019}. The data has high dimensionality, leaving it with $+100$ features after data cleansing and feature engineering. The goal of this task is to predict the total annual compensation.


==> content/data/howtodata.tex <==
\chapter{Evaluating Data for a Research Question}

\input{content/data/intro}
\input{content/data/relatedwork}
\input{content/data/method}
\input{content/data/analysis}
\input{content/data/cases}
\input{content/data/data}
\input{content/data/conclusions}

==> content/data/intro.tex <==
Working with and preparing data for a \emph{short term project research question} can be challenging due to problem-specificity and the short time scales available to prepare the data for analysis and answer a specific set of questions.  In long-term research projects, there is significantly more time and room to explore and adapt the data and the questions. Other factors include the type of question, its potential breadth (e.g., data which is publicly available and has been previously analysed by researchers \citep{kitsios_beyond_2019, concilio_empowering_2017}), datasets from a company with no or limited prior analysis \citep{nolte_you_2018, nolte_touched_2019}, or working with multiple data sources and formats. To effectively incorporate (varied) data, there is a need to have standardised processes and definitions that can account for the complexity and challenges that arise during the data selection and preparation process. In particular, our paper differentiates and focuses on the following data-related dimensions:  appropriateness, readiness, reliability, sensitivity and sufficiency. Our main contributions are as follows:
\begin{itemize}
    
    \item Introduce a framework to analyse the data intended for research questions from several dimensions: appropriateness, readiness, reliability, sensitivity, and sufficiency.

    \item Share insights and experiences from organising datathons with external organisations, mapping 10 data challenges and organisations to the proposed framework.\carlos{rewrite}

    \item Provide recommendations and best practices for organisers to effectively select, prepare, and categorise data for datathon challenges.\carlos{rewrite}
    
\end{itemize}


==> content/data/method.tex <==
\section{Data Study Groups}\label{sec:methdology}
% \subsection{Data Study Groups}

Data Study Groups (DSGs) are an award-winning\footnote{https://www.praxisauril.org.uk/news-policy/blogs/turing-data-study-groups-ke-award-winners} collaborative datathon event organised by The Alan Turing Institute, the UK's national institute for data science and artificial intelligence. Each DSGs consist of multiple datathons (or \enquote{challenges}), typically 3-4, that are worked on collaboratively by a single team (rather than multiple teams competing with each other). The aim of DSGs is to provide opportunities for organisations and participants from academia and industry to work together to solve real-world challenges using data science and ML methodologies. The DSGs are managed and prepared by a specialised internal team of event organisers and interdisciplinary academic support staff.

The events typically run for a week, during which 8-12 participants work in teams to explore and investigate the challenges. The events are overseen by experienced researchers that act as \enquote{principal investigators} (PI) and \enquote{challenge owners} as subject-matter experts. Both provide technical guidance and support for the teams during the week. DSGs have tackled various challenges across different sectors, such as healthcare, finance, and transportation. Figure \ref{fig:analysis} shows the breadth of challenges undertaken, with $\geq 69$ challenge owners spanning $\geq77$ datathons across different domains. Note that we have carried out over 80 datathons, but not all datathons have available meta-data for analysis. 

\begin{figure*}[ht]
\centering
\includegraphics[width=.8\textwidth]{content/data/images/owner_bar.pdf}
\includegraphics[width=.8\textwidth]{content/data/images/domain_pie.pdf}
\caption{Above: Bar chart showing the distribution of sectors from the challenge owners $(n=69)$. Below: Distribution of datathon topics $(N=77)$ for the Data Study Groups (DSGs).}\label{fig:analysis}
\end{figure*} 

During the datathon, a technical report is written by the participants, and edited by the PI after the event. The report collates the work that was carried out by the datathon team and articulates successes, challenges, and recommendations for future analysis directions. The report is not intended to undergo a traditional academic peer-review process to assess novelty. Rather, members of the DSG team at the Alan Turing Institute review the report for scientific rigour and clarity before publication.

The internal peer-review process is aligned with  considerations of responsible research and innovation. DSG challenges hosted at the Turing are all assessed for ethical considerations following guidance published by the Public Policy team \citep{leslie_david_2019_3240529}, therefore, ethics is not an additional data dimension in our process, it is a separate step that is comparable in size to data assessment. Although we recommend that all datathon projects be assessed for data protection and ethical considerations, these processes are outside this paper's scope, as it varies by country, organising institution and partners  needing for an in-depth discussion even within fields to be useful. Our data assessment framework complements institutional policies and can fit within data governance laws across different countries.




==> content/data/relatedwork.tex <==
\section{Related Work}\label{sec:relatedwork}

\subsection{Hackathons \& Datathons}\label{sec:relatedword.hackathons}

Previous research on hackathons has provided valuable insights that can enhance one's understanding of datathons and their effects on organisations and participants. 
Extensive literature reviews include~\cite{Chau2023, Olesen2020}. \cite{Chau2023} found that hackathon and datathon research tends to focus on four core areas: the event purpose, the event format, the processes undertaken and experienced by stakeholders, and the event outcomes (with some papers having more than one focus). They also add that most publications about processes focus on what happens during the event (e.g., intra-team dynamics in collaboration and project brainstorming) rather than before or after. 



%Prior research has covered various aspects of hackathons. For example, Trainer et al. \citep{DBLP:conf/cscw/TrainerKCH16} conducted case studies highlighting the importance of face-to-face interactions and social ties. Olesen et al. \citep{DBLP:conf/chi/OlesenKH21} analysed different hackathon formats and explored the causal relationships between input, process, and effects. Falk et al. \citep{falk_olesen_10_2020} investigated the impact of event structure on learning and research processes. Nolte et al. \citep{DBLP:journals/pacmhci/NolteCH20} emphasized the significance of sustainability and continuity in hackathon projects. Kollwitz et al. \citep{kollwitz_what_2019} developed taxonomies of hackathon design decisions related to operational requirements and strategic goals.



%Other works such as \citet{DBLP:journals/cacm/GebruMVVWDC21,DBLP:conf/fat/MitchellWZBVHSR19} introduce documentation for datasets and models, aiming to enhance transparency and accountability in data and model usage. In contrast, our paper offers clear guidelines and best practices to effectively handle data in the context of datathons, explicitly emphasising the complexities and challenges unique to collaborative data-driven hackathon events.


As mentioned in the introduction, datathons are data science or data-centric hackathons. The work in \cite{Anslow2016} explores how these can enhance data science curriculum (e.g., through improved data science, communication, and community engagement skills) and that in~\cite{Kuter2020} on how to run a datathon with very limited resources.
%In the context of datathons, 
\cite{doi:10.1126/scitranslmed.aad9072} focus on healthcare and emphasize the cross-disciplinary aspects of datathons, 
%as cross-domain activities, 
claiming they help address poor study design, paucity of data, and improve analytical rigour through increased transparency. \cite{luo_mit_2021} conducted a virtual datathon focusing on the early stages of the Covid-19 pandemic, highlighting the importance of interdisciplinary and diverse team compositions. \cite{piza_assessing_2018} found a significant association between positive teamworking behaviors and affective learning in a healthcare-focused datathon, pointing out effective leadership as the key factor. 

We propose to add to existing literature that explores challenges and best practices in datathons, with a focus on data practices. More specifically, and following the terminology in~\cite{Chau2023}, we focus on data as a ``technical project material'' in datathon formats, and examine key challenges that can arise in data evaluation and preparation during the ``pre-hackathon'' organisation process. To the best of our knowledge, prior research has not focused on data-related challenges in the specific context of datathons. 


\subsection{Data Analysis Dimensions}

Previous research on data quality evaluation has focused on general description frameworks and metrics, rather than datathon context-specific development of methods~\citep{wang1996beyond, zaveri2016quality, juran1974quality, schlegel2020methodological}.


Early work in the area \citep{wang1996beyond} presented a conceptual framework for assessing \enquote{data quality} (i.e. assessing issues that can affect the potentiality of the applications that use the data),
%\citep{zaveri2016quality}, 
which included 15 dimensions grouped under
four categories: intrinsic; contextual; representational and system-supported. 
Indeed, ``data quality'' is commonly viewed as a multi-dimensional construct that defines ``fitness of use'' and may depend on various factors \citep{zaveri2016quality, juran1974quality}, such as believability, accuracy, completeness, relevancy, objectivity, accessibility, amongst several others \citep{wang1996beyond}. The context-specific methodology of \cite{schlegel2020methodological} focuses on defect diagnosis and prediction and addresses the following five dimensions, which they argued were the most important for assessing \enquote{data quality} (which they rather refer to as \enquote{data suitability}): relevancy; completeness; appropriate amount (of data); accessibility and interpretability. Their study focused on developing guidance for companies, using various metrics and evaluation levels, on how to gain insight into the suitability of the data collected in the context of defect diagnosis and prediction. Our work extends and builds upon these previous frameworks and methodologies by applying them specifically to the challenges and requirements of datathons. In particular, we consider the five following dimensions in the context of data-driven problem-solving during the datathon events: data appropriateness, readiness, reliability, sensitivity and sufficiency. In what follows, we link our proposed dimensions to existing terminology in \cite{wang1996beyond} and \cite{schlegel2020methodological} where possible, and mention other related research in the field. 

\textbf{Appropriateness:} This dimension considers the question \enquote{Is the data relevant to the data science questions posed (i.e., problem-specific)?}, and closely aligns with  \enquote{relevancy} \citep{wang1996beyond, schlegel2020methodological}. Examples of context-specific uses of relevancy include \cite{Daly_2006}, which provide a comprehensive set of guidelines for analysing specific climate datasets. In their guidelines, the authors outline the relevancy of specific climate factors for different types of analysis, and \cite{schlegel2020methodological} provides domain-specific concepts to assess data suitability along the production chain for defect prediction.%\citep{DBLP:journals/fgcs/ArdagnaCSV18} propose a data quality methodology based on user requirements such as  time   minimization, confidence maximization, and budget minimization. In this work we distinguish between five dimensions of data and discuss them within the context of data in datathons.


\textbf{Readiness:} This dimension considers the questions \enquote{Is the data analysis-ready?}, and includes \enquote{completeness} and \enquote{accessibility}
%, \enquote{accuracy},  %\enquote{interpretability}, and %\enquote{consistency} 
\citep{wang1996beyond, schlegel2020methodological}. Technology readiness levels~\citep{dunbar2017technology,hirshorn2017nasa} was developed in the 1970s as a standardized technology maturity assessment tool in the aerospace engineering sector. NASA developed a scale with multiple degrees which has increased from 7, in the early years~\citep{sadin1989nasa}, up to 15 degrees in the latest reviews~\citep{DBLP:journals/se/OlechowskiEJT20}.

Similarly,~\cite{DBLP:journals/corr/Lawrence17} proposed the use of data readiness levels, giving  a rough outline of the stages of data preparedness and speculating on how formalization of these levels into a common language could facilitate project management. Building on this previous work, we specify four data readiness levels but specifically within the context of datathons challenges.

\cite{Afzal2021} outlines a recommended task-agnostic `Data Readiness Report' template for a project's lifecycle, which includes different stakeholders involved such as final contributions by data scientists.
\cite{Castelijns2020} identifies 3 levels of data readiness and introduces \texttt{PyWash}, which is a semi-automatic data cleaning and processing \texttt{Python} package. Their levels also include a series of steps which includes feature processing and cleaning. In their works, the use of `data readiness' refers to the end-to-end lifecycle of a data science project, including steps typically taken during a datathon and after. Other works focus specifically on `big data' readiness and in country-specific ecosystems which may not be easily extendable \citep{austin2018path,joubert2023measuring,hu2016readiness,zijlstra2017open,romijn2014using}. Since datathons are not confined to a single use-case, we believe it would be more appropriate to create a framework that can work across different applications. 


\textbf{Reliability:} This dimension considers the question \enquote{How biased is the data?}, and includes \enquote{objectivity} \citep{wang1996beyond}. The reliability of data is crucial for AI applications as it directly impacts the accuracy and fairness of the outcomes. Biased data which does not represent the problem fairly returns unreliable results \citep{DBLP:journals/widm/NtoutsiFGINVRTP20}. Drawing from established frameworks such as \cite{Suresh2019} and \cite{DBLP:journals/widm/NtoutsiFGINVRTP20}, we identify several potential sources of bias that can undermine the reliability of the data. Selected examples may include: \emph{(i)} historical bias, which arises from past societal or systemic inequalities; \emph{(ii)} representation bias, where certain groups or perspectives are underrepresented in the data; \emph{(iii)} measurement bias, which stems from flawed or subjective data collection methods; and \emph{(iv)} aggregation bias, which occurs when data is combined or summarised in a way that does not accurately represent each sub-group within the wider population.


\textbf{Sensitivity:} This dimension considers the questions \enquote{How sensitive is the data?}. We build on existing work from~\cite{DBLP:journals/corr/abs-1908-08737} by incorporating their data sensitivity analysis categorisation to our framework. They propose a defined tier-based system for sensitive data management in the cloud, which contain: \emph{tier 0}, datasets with no personal information or data which carries legal, reputational, or political risks; \emph{tier 1}, data that can be analysed on personal devices or data that can be published in the future without significant risks, such as anonymised or synthetic information; \emph{tier 2}, data that is not linked directly to personal information, but may derive from it through synthetic generation or pseudonymisation; \emph{tier 3}, data that presents a risk to personal safety, health, or security on disclosure. This may include pseudonymous or generated data with weak confidence in the anonymisation mechanism or commercially and legally confidential material; \emph{tier 4}, personal information that poses a substantial threat to personal safety, commercial, or national security and is likely to be subject to attack.

The data used in the study may also need to adhere to various regulations, including but not limited to the Data Protection Act~\citep{ukdpa2018}, GDPR~\citep{european_commission_regulation_2016}, and specific regulations governing special categories of data \citep{ico_guidance, nis_directive}. Additionally, different countries or sectors may have their own specific regulations in place. It is important to note that the application of these laws is evaluated on a case-by-case basis, and this paper does not provide specific guidance on how to comply with them.


\textbf{Sufficiency:}
This dimension considers the question \enquote{How much data is enough data for a given datathon?}, and includes \enquote{appropriate amount}~\citep{wang1996beyond, schlegel2020methodological}.
%\carlos{This section is controversial and too long.}
This question is highly problem and method-specific, and 
%The question 
has been formulated in many research fields. In an early study, \cite{Lauer1995} explored a series of issues in analysing data requirements for statistical Natural Language Processing (NLP) systems and suggested the first steps toward a theory of data requirements. Questions such as (i) "
\enquote{Given a limited amount of training data, which methods are more likely to be accurate?}, or (ii) \enquote{Given a particular method, when will acquiring further data stop to improve predictive accuracy?}, were addressed. In intelligent vehicles, \cite{Wang2017} proposed a general method to determine the appropriate data model driver behavior from a statistical perspective. They point out that this question has not been fully explored in their field of research, but it is highly relevant given that insufficient data leads to inaccurate models, while excessive data can result in high costs and a waste of resources. \cite{Cho2015} presented a general methodology for determining the size of the training dataset necessary to achieve a certain classification accuracy in medical image deep learning systems. They employed the \textit{learning curve} method \citep{Figueroa2012}, which models classification performance as a function of the training sample size. They pointed out that, in medical image deep learning, data scarcity is a relevant problem. Developing a methodology to estimate how large a training sample needs to be in order to achieve a target accuracy is therefore highly relevant. Since datathons include a wide range of applications and approaches, we adopt a different take on \enquote{sufficiency} and propose general guidelines based on experiences in prior datathons. In our case studies, we make case-specific observations (see section~\ref{sec:casestudies}).

==> content/equalTreatment/conclusions.tex <==
\section{Conclusions}
We introduced a novel approach for fairness in machine learning by measuring \emph{equal treatment}. While related work
employed model predictions to judge  \emph{equal outcomes}, our measure of {equal treatment} is more fine-grained, accounting for the usage of attributes by the model via explanation distributions. Consequently, {equal treatment} implies {equal outcomes}, but the converse is not necessarily true. 

This paper also seeks to improve the understanding of how theoretical concepts of fairness from liberalism-oriented political philosophy align with technical measurements. Our measure of equal treatment diverges from a naive understanding of liberalism. When one demographic group is structurally disadvantaged compared to another group, our measure of equal treatment will pick this up via all the non-protected attributes that are proxies for protected characteristics. Therefore, our measure of equal treatment is much more nuanced than approaches that would oversimplify by only ignoring protected attributes. Implications warrant further techno-philosophical discussions.

%\steffen{We should note that truly equal treatment, such as measured by us, is nearly impossible to achieve because our measure also considers the structural differences between demographic  groups. Therefore, the machine learning aim can rarely be to achieve perfect equal treatment, but rather an improvement towards better equal treatment measures, such as illustrated by our experiments.}\steffen{My last comment may be too hard to understand without reference to the university admissions example that we discussed, Carlos. In this fictitious example, there is only one non-protected attribute (SAT score), demographic group 1 scored a SAT below 1500, and demographic group 2 scored a SAT above 1500; 1500 is the college admission boundary. The non-protected attribute is a perfect proxy, and the only way to achieve equal treatment as measured by us is to ignore the SAT score. This is not exactly what radical liberalists would suggest. Still, it is the consequent implementation of not looking at demographic status --- which is only possible if proxy attributes of demographic status are also discarded.}
%\steffen{A discussion, like this, in conclusion, would tie the knot between the beginning and the end of our paper.}

\textbf{Limitations:}
Political philosophical notions of distributive justice are more complex than we can account for in this paper.
Our research has focused on tabular data using Shapley values, which allow for theoretical guarantees but may differ from their computational approximations. 
%open to multiple interpretations from different angles. While our results are promising, it's essential to acknowledge that our research is centered around tabular data and is based on Shapley values, which provide theoretical guarantees that may differ from the SHAP approximation (a computational approach). 
It is possible that alternative AI explanation techniques, such as feature attribution methods, logical reasoning, argumentation, or counterfactual explanations, could be useful and offer their unique advantages to definitions of equal treatment. It is important to note that employing fair AI techniques does not necessarily ensure fairness in socio-technical systems based on AI, as stated in~\cite{DBLP:conf/fat/KulynychOTG20}.


==> content/expShift/appExperiments.tex <==
\section{Further Experiments on Real Data}\label{app:real.data}
In this section, we extend the prediction task of the main body of the paper.  The methodology used follows the same structure. We start by creating a distribution shift by training the model $f_\theta$ in California in 2014 and evaluating it in the rest of the states in 2018, creating a geopolitical and temporal shift. The model $g_\theta$ is trained each time on each state using only the $X^{New}$ in the absence of the label, and its performance is evaluated by a 50/50 random train-test split. As models, we use a gradient boosting decision tree\cite{xgboost,catboost} as estimator $f_\theta$, approximating the Shapley values by TreeExplainer \cite{lundberg2020local2global}, and using logistic regression for the \textit{Explanation Shift Detector}.



\subsection{ACS Employment}
The objective of this task is to determine whether an individual aged between 16 and 90 years is employed or not. The model's performance was evaluated using the AUC metric in different states, except PR18, where the model showed an explanation shift. The explanation shift was observed to be influenced by features such as Citizenship and Military Service. The performance of the model was found to be consistent across most of the states, with an AUC below 0.60. The impact of features such as difficulties in hearing or seeing was negligible in the distribution shift impact on the model. The left figure in Figure \ref{fig:xai.employment.shift} compares the performance of the Explanation Shift Detector in different states for the ACS Employment dataset.

\begin{figure*}[ht]
\centering
\includegraphics[width=.49\textwidth]{content/expShift/images/AUC_OOD_ACSEmployment.pdf}\hfill
\includegraphics[width=.49\textwidth]{content/expShift/images/feature_importance_ACSEmployment.pdf}
\caption{The left figure shows a comparison of the performance of the Explanation Shift Detector in different states for the ACS Employment dataset. The right figure shows the feature importance analysis for the same dataset.}
\label{fig:xai.employment.shift}
\end{figure*}

Additionally, the feature importance analysis for the same dataset is presented in the right figure in Figure \ref{fig:xai.employment.shift}.
\subsection{ACS Travel Time}

The goal of this task is to predict whether an individual has a commute to work that is longer than $+20$ minutes. For this prediction task, the results are different from the previous two cases; the state with the highest OOD score is $KS18$, with the \enquote{Explanation Shift Detector} highlighting features as Place of Birth, Race or Working Hours Per Week. The closest state to ID is CA18, where there is only a temporal shift without any geospatial distribution shift.
\begin{figure*}[ht]
\centering
\includegraphics[width=.49\textwidth]{content/expShift/images/AUC_OOD_ACSTravelTime.pdf}\hfill
\includegraphics[width=.49\textwidth]{content/expShift/images/feature_importance_ACSTravelTime.pdf}
\caption{In the left figure, comparison of the performance of \textit{Explanation Shift Detector}, in different states for the ACS TravelTime prediction task.  In the left figure, we can see how the state with the highest OOD AUC detection is KS18 and not PR18 as in other prediction tasks; this difference with respect to the other prediction task can be attributed to \enquote{Place of Birth}, whose feature attributions the model finds to be more different than in CA14.}
\label{fig:xai.traveltime.shift}
\end{figure*}


\subsection{ACS Mobility}
The objective of this task is to predict whether an individual between the ages of 18 and 35 had the same residential address as a year ago. This filtering is intended to increase the difficulty of the prediction task, as the base rate for staying at the same address is above $90\%$ for the population \cite{ding2021retiring}.

The experiment shows a similar pattern to the ACS Income prediction task (cf. Section \ref{fig:xai.income.shift}), where the inland US states have an AUC range of $0.55-0.70$, while the state of PR18 achieves a higher AUC. For PR18, the model has shifted due to features such as Citizenship, while for the other states, it is Ancestry (Census record of your ancestors' lives with details like where they lived, who they lived with, and what they did for a living) that drives the change in the model.

As depicted in Figure \ref{fig:xai.mobility.shift}, all states, except for PR18, fall below an AUC of explanation shift detection of $0.70$. Protected social attributes, such as Race or Marital status, play an essential role for these states, whereas for PR18, Citizenship is a key feature driving the impact of distribution shift in model.

\begin{figure*}[ht]
\centering
\includegraphics[width=.49\textwidth]{content/expShift/images/AUC_OOD_ACSMobility.pdf}\hfill
\includegraphics[width=.49\textwidth]{content/expShift/images/feature_importance_ACSMobility.pdf}
\caption{Left figure shows a comparison of the \textit{Explanation Shift Detector}'s performance in different states for the ACS Mobility dataset. Except for PR18, all other states fall below an AUC of explanation shift detection of $0.70$. The features driving this difference are Citizenship and Ancestry relationships. For the other states, protected social attributes, such as Race or Marital status, play an important role.}
\label{fig:xai.mobility.shift}
\end{figure*}

\subsection{StackOverflow Survey Data: Novel Covariate Group}

This experimental section evaluates the proposed Explanation Shift Detector approach on real-world data under novel group distribution shifts. In this scenario, a new unseen group appears at the prediction stage, and the ratio of the presence of this unseen group in the new data is varied. The estimator used is a gradient-boosting decision tree or logistic regression, and a logistic regression is used for the detector. The results show that the AUC of the Explanation Shift Detector varies depending on the quantification of OOD explanations, and it show more sensitivity w.r.t. to model variations than other state-of-the-art techniques.

The dataset used is the StackOverflow annual developer survey has over 70,000 responses from over 180 countries examining  aspects of the developer experience~\cite{so2019}. The data has high dimensionality, leaving it with $+100$ features after data cleansing and feature engineering. The goal of this task is to predict the total annual compensation.

\begin{figure}[ht]
\centering
\includegraphics[width=.49\textwidth]{content/expShift/images/NewCategoryHyperSO.pdf}\hfill
\includegraphics[width=.49\textwidth]{content/expShift/images/NewCategoryHyperXGBSO.pdf}
\caption{Both images represent the AUC of the \textit{Explanation Shift Detector} for different countries on the StackOverflow survey dataset under novel group shift. In the left image, the detector is a logistic regression, and in the right image, a gradient-boosting decision tree classifier. By changing the model, we can see that low-complexity models  are unaffected by the distribution shift, while when increasing the model complexity, the out-of-distribution model behaviour starts to be tangible}
\label{fig:xai.hyperSO.shift}
\end{figure}


\section{Experiments with Modeling Methods and Hyperparameters}\label{app:modelingmethods}
In the next sections, we are going to show the sensitivity or our method to variations of  the estimator $\textcolor{magenta}{f}$, the detector $\textcolor{magenta}{g}$, and the parameters of the estimator $f\textcolor{magenta}{_\theta}$. 

As an experimental setup, In the main body of the paper, we have focused on the UCI Adult Income dataset. The experimental setup has been using Gradient Boosting Decision Tree as the original estimator $f_\theta$ and then as \enquote{Explanation Shift Detector} $g_\psi$ a logistic regression. In this section, we extend the experimental setup by providing experiments by varying the types of algorithms for a given experimental set-up: the UCI Adult Income dataset using the Novel Covariate Group Shift for the \enquote{Asian} group with a fraction ratio of $0.5$ (cf. Section \ref{sec:experiments}).
\subsection{Varying Estimator and Explanation Shift Detector}\label{app:varying}


OOD data detection methods based on input data distributions only depend on the type of detector used, being independent of the estimator. OOD Explanation methods rely on both the model and the data. Using explanations shifts as indicators for measuring distribution shifts impact on the model enables us to account for the influencing factors of the explanation shift. Therefore, in this section, we compare the performance of different types of algorithms for explanation shift detection  using the same experimental setup. The results of our experiments show that using Explanation Shift enables us to see differences in the choice of the original estimator $f_\theta$ and the Explanation Shift Detector $g_\phi$


\begin{table}[ht]
\begin{tabular}{cccccccc}
\multicolumn{1}{l}{}                       & \multicolumn{7}{c}{Estimator $f_\theta$}                                                                                                         \\ \cline{2-8} 
\multicolumn{1}{c|}{Detector $g_\phi$}              & \textbf{XGB} & \textbf{Log.Reg} & \textbf{Lasso} & \textbf{Ridge} & \textbf{Rand.Forest} & \textbf{Dec.Tree} & \textbf{MLP} \\ \hline
\multicolumn{1}{c|}{\textbf{XGB}}          & 0.583        & 0.619                 & 0.596          & 0.586          & 0.558                 & 0.522                 & 0.597        \\
\multicolumn{1}{c|}{\textbf{LogisticReg.}} & 0.605        & 0.609                 & 0.583          & 0.625          & 0.578                 & 0.551                 & 0.605        \\
\multicolumn{1}{c|}{\textbf{Lasso}}        & 0.599        & 0.572                 & 0.551          & 0.595          & 0.557                 & 0.541                 & 0.596        \\
\multicolumn{1}{c|}{\textbf{Ridge}}        & 0.606        & 0.61                  & 0.588          & 0.624          & 0.564                 & 0.549                 & 0.616        \\
\multicolumn{1}{c|}{\textbf{RandomForest}} & 0.586        & 0.607                 & 0.574          & 0.612          & 0.566                 & 0.537                 & 0.611        \\
\multicolumn{1}{c|}{\textbf{DecisionTree}} & 0.546        & 0.56                  & 0.559          & 0.569          & 0.543                 & 0.52                  & 0.569       
\end{tabular}
\caption{Comparison of explanation shift detection performance, measured by AUC, for different combinations of explanation shift detectors and estimators on the UCI Adult Income dataset using the Novel Covariate Group Shift for the \enquote{Asian} group with a fraction ratio of $0.5$ (cf. Section \ref{sec:experiments}). The table shows that the choice of detector and estimator can impact the OOD explanation performance.  We can see how, for the same detector, different estimators flag different OOD explanations performance. On the other side, for the same estimators, different detectors achieve different results.}\label{tab:benchmark}
\end{table}

\subsection{Hyperparameters Sensitivity Evaluation}\label{app:hyperparameter.shift}
This section presents an extension to our experimental setup where we vary the model complexity by varying the model hyperparameters $\Ss(f\textcolor{magenta}{_\theta},X)$. Specifically, we use the UCI Adult Income dataset with the Novel Covariate Group Shift for the \enquote{Asian} group with a fraction ratio of $0.5$ as described in Section \ref{sec:experiments}.

In this experiment, we changed the hyperparameters of the original model: for the decision tree, we varied the depth of the tree, while for the gradient-boosting decision,  we changed the number of estimators, and for the random forest, both hyperparameters. We calculated the Shapley values using TreeExplainer \cite{lundberg2020local2global}. For the Detector choice of model, we compare Logistic Regression and XGBoost models.


\begin{figure}[ht]
\centering
\includegraphics[width=.49\textwidth]{content/expShift/images/NewCategoryHyper.pdf}\hfill
\includegraphics[width=.49\textwidth]{content/expShift/images/NewCategoryHyperXGB.pdf}
\caption{Both images represent the AUC of the \textit{Explanation Shift Detector}, in different states for the ACS Income dataset under novel group shift. In the left image, the detector is a logistic regression, and in the right image, a gradient-boosting decision tree classifier. By changing the model, we can see that vanilla models (decision tree with depth 1 or 2) are unaffected by the distribution shift, while when increasing the model complexity, the out-of-distribution impact of the data in the model  starts to be tangible}
\label{fig:xai.hyper.shift}
\end{figure}


The results presented in Figure \ref{fig:xai.hyper.shift} show the AUC of the \textit{Explanation Shift Detector} for the ACS Income dataset under novel group shift. We observe that the distribution shift does not affect very simplistic models, such as decision trees with depths 1 or 2. However, as we increase the model complexity, the out-of-distribution data impact on the model becomes more pronounced. Furthermore, when we compare the performance of the \textit{Explanation Shift Detector} across different models, such as Logistic Regression and Gradient Boosting Decision Tree, we observe distinct differences(note that the y-axis takes different values).

In conclusion, the explanation distributions serve as a projection of the data and model sensitive to what the model has learned. The results demonstrate the importance of considering model complexity under distribution shifts.





\section{LIME as an Alternative Explanation Method}\label{app:LIME}
Another feature attribution technique that satisfies the aforementioned properties (efficiency and uninformative features Section~\ref{sec:xai.foundations}) and can be used to create the explanation distributions is LIME (Local Interpretable Model-Agnostic Explanations). The intuition behind LIME is to create a local interpretable model that approximates the behavior of the original model in a small neighbourhood of the desired data to explain~\cite{ribeiro2016why,ribeiro2016modelagnostic} whose mathematical intuition is very similar to the Taylor series. In this work, we have proposed explanation shifts as a key indicator for investigating the impact of distribution shifts on ML models. In this section, we compare the explanation distributions composed by SHAP and LIME methods. LIME can potentially suffers several drawbacks: 

\begin{itemize}
    \item \textbf{Computationally Expensive:} Its currently implementation is more computationally expensive than current SHAP implementations such as TreeSHAP~\cite{lundberg2020local2global}, Data SHAP \cite{DBLP:conf/aistats/KwonRZ21,DBLP:conf/icml/GhorbaniZ19} or Local  and Connected SHAP~\cite{DBLP:conf/iclr/ChenSWJ19}, the problem increases when we produce explanations of distributions. Even though implementations might be improved, LIME requires sampling data and fitting a linear model which is a computationally more expensive approach than the aforementioned model-specific approaches to SHAP.
    
    \item \textbf{Local Neighborhood:} The definition of a local \enquote{neighborhood}, which can lead to instability of the explanations. Slight variations of this explanation hyperparameter lead to different local explanations. In \cite{DBLP:conf/aies/SlackHJSL20} the authors showed that the explanations of two very close points can vary greatly. 

    \item \textbf{Dimensionality:} LIME requires as a hyperparameter the number of features to use for the local linear approximation. This creates a dimensionality problem as for our method to work, the explanation distributions have to be from the exact same dimensions as the input data. Reducing the number of features to be explained might improve the computational burden.

\end{itemize}



\begin{figure}[ht]
\centering
\includegraphics[width=.49\textwidth]{content/expShift/images/SOTAsensitivityLime.pdf}\hfill
\includegraphics[width=.49\textwidth]{content/expShift/images/NewCategoryLime.pdf}
\caption{Comparison of the explanation distribution generated by LIME and SHAP. The left plot shows the sensitivity of the predicted probabilities to multicovariate changes using the synthetic data experimental setup of \ref{fig:sensitivity} on the main body of the paper. The right plot shows the distribution of explanation shifts for a New Covariate Category shift (Asian) in the ASC Income dataset.}
\label{fig:lime}
\end{figure}

Figure \ref{fig:lime} compares the explanation distributions generated by LIME and SHAP. The left plot shows the sensitivity of the predicted probabilities to multicovariate changes using the synthetic data experimental setup from Figure \ref{fig:sensitivity} in the main body of the paper. The right plot shows the distribution of explanation shifts for a New Covariate Category shift (Asian) in the ASC Income dataset. The performance of OOD explanations detection is similar between the two methods, but LIME suffers from two drawbacks: its theoretical properties rely on the definition of a local neighborhood, which can lead to unstable explanations (false positives or false negatives on explanation shift detection), and its computational runtime required is much higher than that of SHAP (see experiments below).


\subsection{Runtime}
We conducted an analysis of the runtimes of generating the explanation distributions using the two proposed methods. The experiments were run on a server with 4 vCPUs and 32 GB of RAM. We used \texttt{shap} version $0.41.0$ and \texttt{lime} version $0.2.0.1$ as software packages. In order to define the local neighborhood for both methods in this example we use all the data provided as background data. As an estimator, we use an xgboost and compare the results of TreeShap against LIME.  When varying the number of samples we use 5 features and while varying the number of features we use $1000$ samples.


\begin{figure}[ht]
\centering
\includegraphics[width=.49\textwidth]{content/expShift/images/computational_samples.pdf}\hfill
\includegraphics[width=.49\textwidth]{content/expShift/images/computational_features.pdf}
\caption{Wall time for generating explanation distributions using SHAP and LIME with different numbers of samples (left) and different numbers of columns (right). Note that the y-scale is logarithmic. The experiments were run on a server with 4 vCPUs and 32 GB of RAM. The runtime required to create an explanation distributions with LIME is far greater than SHAP for a gradient-boosting decision tree}
\label{fig:computational}
\end{figure}

Figure \ref{fig:computational}, shows the wall time required for generating explanation distributions using SHAP and LIME with varying numbers of samples and columns. The runtime required of generating an explanation distributions using LIME is much higher than using SHAP, especially when producing explanations for distributions. This is due to the fact that LIME requires training a local model for each instance of the input data to be explained, which can be computationally expensive. In contrast, SHAP relies on heuristic approximations to estimate the feature attribution with no need to train a model
for each instance. The results illustrate that this difference in computational runtime becomes more pronounced as the number of samples and columns increases. 

We note that the computational burden of generating the explanation distributions can be further reduced by limiting the number of features to be explained, as this reduces the dimensionality of the explanation distributions, but this will inhibit the quality of the explanation shift detection as it won't be able to detect changes on the distribution shift that impact model on those features.


Given the current state-of-the-art of software packages we have used SHAP values due to lower runtime required and that theoretical guarantees hold with the implementations. In the experiments performed in this paper, we are dealing with a medium-scaled dataset with around $\sim 1,000,000$ samples and $20-25$ features. Further work can be envisioned on developing novel mathematical analysis and software that study under which conditions which method is more suitable.




==> content/mysc.tex <==


\subsection{Uncertainty}

Uncertainty refers to the lack of knowledge about the model predictions. While there are many sources of uncertainty, there has been a clear differentiation between two types of uncertainty: aleatoric (indirect), inherent randomness on the model input, and epistemic (direct), absence of enough data during the learning process. However, attempts to get a hold of the two concepts might seem slippery in many situations ~\cite{aleatory_epistemic,Gal2016Uncertainty,epistemic_uncertainty}.


When using machine learning models, information about the uncertainty of their predictions, or predictive uncertainty, is essential in decision making~\cite{bhatt2021uncertainty,desiderataECB}. Uncertainty quantification supports the decision process in many areas such as nuclear security, risk management, healthcare, or finance, where decisions at the scale of billions of dollars~\cite{need_for_uncertainty}. Uncertainty is characterized differently depending on the task. 

For regression tasks, uncertainty is often expressed in terms of error bars. For example, when predicting the crime count of a country, one can predict that the number of predicted crimes is $1468\pm 20$, where
\enquote{$\pm 20$} represents a $95\%$ confidence interval. 

For classification tasks, it can also be applied. For example, a medical doctor,aware of the traumatic cost of an operation, will only decide to operate on a patient if there is enough evidence of cancer diagnostic and the disappearance of the illness compensates the effects of the operation. In this scenario, a prediction such as \enquote{there is 99\% probability of cancer} is fundamentally different from \enquote{there is 55\% probability of cancer}

Uncertainty estimation is being developed at a fast pace. Model averaging ~\cite{kumar2012bootstrap,gal2016dropout,lakshminarayanan2017simple,arnez2020} has emerged as the most common approach to uncertainty estimation. Ensemble and sampling-based uncertainty estimates have been successfully applied to many use cases such as detecting misclassifications~\cite{unc_ood_class}, out-of-distribution inputs~\citep{dangelo2021uncertaintybased}, adversarial attacks ~\cite{adversarialUncertainty,smith2018understanding}, automatic language assessments~\cite{malinin2019uncertainty} and active learning~\cite{kirsch2019batchbald}.



Knowledge about the uncertainty of the predictions can be a powerful tool to detect model discrimination, improve decision-making, build trust or evaluate machine learning model performance.



\subsection{Counterfactual reasoning}

A counterfactual explanation describes a situation in the form: \enquote{If X had not occurred, Y would have occurred}. One example can be: \enquote{If I hadn't gone swimming in cold water, I wouldn't be sick}. The event of being sick is caused by swimming in cold water. Counterfactuals reasoning is a representation of alternatives to an event and produces consequences that can be both beneficial and aversive~\cite{roese1997counterfactual}.

The explanation offered through this understanding supports can support different users. For instance, when data is identified to belong to a particular class, providing a set of actionable changes that would lead to a different decision can assist an expert in correcting or modifying the data. 

Counterfactual generation aims to address this issue by proposing to the \emph{business experts} \emph{the minimal feasible change in the data in order to change the output of the algorithm}. Such a process enhances the experts' understanding (and might further foster trust in the system). We formulate the problem following the counterfactual recourse formulation by Utsun et~al.~\cite{utsun_linear_recourse,ActionableRecouserLinear,AlgRecourse_Counterfactual_Interventions} 

\begin{equation} \label{eq:counterfactual}
\delta^{*} \in \texttt{argmin} \quad cost(\delta: x^{F}) \quad s.t. \quad h(x^{CFE}) \neq h(x^F)
\end{equation}
\begin{subequations}
\begin{align}
x^{CFE} = x^F + \delta\\
x^{CFE} \in P, \delta \in F
\end{align} 
\end{subequations}


Where cost $(\cdot; x^F): X x X \rightarrow R_+$ is a user-specified cost that encodes preferences between feasible actions from $x^F$, and $F$ and $P$ are optional sets of feasibility and plausibility constraints, restricting the actions and the resulting counterfactual explanation respectively~\cite{AlgRecourse_Counterfactual_Interventions}. The feasibility constraints, as introduced in~\cite{ActionableRecouserLinear,AlgRecourse_Counterfactual_Interventions} aim at restricting the set of features that the individual may act upon.


\section{Explainable AI}


Improvements in the predictive performance of machine learning algorithms have led to applications across many domains, including central banking, education, healthcare, and public policy. As machine learning becomes increasingly ingrained in society as a means to improve business efficiency and decision-making, it becomes crucial to establish processes for ensuring fairness, explainability, data privacy, and security. 

Explainability has become an important concept in legal and ethical guidelines for data and machine learning applications~\cite{intuitive_appeal}. The European Union General Data Protection Regulation (GDPR)\cite{gdpr} states that individuals have the right to receive an explanation for the output of an automated algorithm~\cite{gdpr_right}. Ensuring algorithmic accountability and transparency in machine learning models is a key ingredient toward understanding how decisions are made by the system. Understanding decisions is a prerequisite to detecting potential bias and ensuring fair and safe machine learning systems. 

The research community has made an enormous effort to design algorithmic methods for explainability. Various publications reconcile the information of all relevant papers, create explainable AI (xAI) taxonomies, define future opportunities and current gaps.~\cite{guidotti_survey,paco_herrera_xai_taxonomi,exaplaining_explanations_ATI,explainabe_public_policy,explaining_explanations_overview_of_interpretability,xai_concepts,rudin2019stop}. In this section we review some of the most used explainability tools.

\subsection{Feature relevance explanations}

Feature attribution or relevance methods try to describe the model predictions as the sum of the feature effects. They can be decomposed into two main approaches: $(i)$ global explanations, describing the average behavior of a machine learning model, or $(ii)$ local explanations, explaining the behavior of a single instance. Particularly in this section, we are going to focus on local feature relevance explanations.

Let $f_\theta$ be a trained and parametrized classification model on $\Dd{tr}$ with parameters $\theta$. Local methods try to ensure that whenever we are in the neighborhood of the instance to explain $z_i \approx x_i \in D^{n}$, the model $g(f_\theta, z) \approx g(f_\theta,x_i)$ ~\cite{Chen2021,shapNIPS2017,shapTree}

\begin{equation}\label{eq:featureRelevance}
    g(f_\theta, D)=\varphi_0+\sum_{i}^n\sum_{j}^m\varphi_{i,j} z_{i,j}
\end{equation}

From the equation above, $\varphi_{i,j} \in \mathbb{R}$ are the feature attribution for a feature $j$ of the instance $i$. Methods with explanation models matching definition \ref{eq:featureRelevance} attribute an effect $\varphi_{i,j}$ to each feature, and aggregating the effects $\varphi_{:,j}$ provides an explanation for $\D(X_{:,j})$~\cite{shapTree}

 One of the most popular approaches to machine learning explainability in recent years has been the use of \textbf{Shapley values} to attribute relevance to features used in the machine learning model~\cite{shapTree,lundberg2017unified}. In this work, we will be focusing on Shapley values as a local feature relevance explainable AI technique. Their usage has been applied in many fields from credit scoring, statistical production systems, model monitoring, time series, social sciences, and central banking. The Shapley value is a concept from coalition game theory that aims to allocate the surplus generated by the grand coalition in a game to each of its players~\cite{shapley}. In a general sense, the Shapley value can be formulated as:
 
 \begin{equation}
     \mathcal{S}_i = \frac{1}{M!}\sum_R [v(\mathbb{S}^R\cup i) - v(\mathbb{S}^R)]
 \end{equation}
 
 Where R is one possible permutation of the order in which the players join the coalitional, $\mathbb{S}^R$ is the set of players joining the coalition before player $i$ and $v:\mathbb{S} \in \mathcal{P}(M) \rightarrow \mathbb{R}^1$ is a coalitional game that maps the power set $\mathbb{P}$ of all players $M$ to a scalar value ~\cite{DBLP:journals/corr/ShapTrueModelTrueData}.


Another local feature relevance explanation has been the usage of local surrogate models such as LIME~\cite{ribeiro2016why,ribeiro2016modelagnostic}, whose algorithmic idea can be quite intuitive. First, let's only consider the already trained black box model without any training data; the model can be queried to make predictions for certain data. By calling the model around the vicinity of a certain instance many times, we can create a new training dataset that resembles the original model around a local area. By fitting any explainable model such as a linear estimator or a decision tree~\cite{lore} on this perturbed data. The learned model can be a good approximation of the machine learning model predictions locally, but it will not be a good global approximation. This kind of accuracy is also called local fidelity~\cite{christoph_molnar2019_interpretableML}.








==> content/selectiveRegression/main.tex <==
\chapter{Building Indicators of Model Performance Deterioration}

